Distributed Hybrid Power State Estimation under PMU Sampling Phase Errors

Phasor measurement units (PMUs) have the advantage of providing direct measurements of power states. However, as the number of PMUs in a power system is limited, the traditional supervisory control and data acquisition (SCADA) system cannot be replaced by the PMU-based system overnight. Therefore, hybrid power state estimation taking advantage of both systems is important. As experiments show that sampling phase errors among PMUs are inevitable in practical deployment, this paper proposes a distributed power state estimation algorithm under PMU phase errors. The proposed distributed algorithm only involves local computations and limited information exchange between neighboring areas, thus alleviating the heavy communication burden compared to the centralized approach. Simulation results show that the performance of the proposed algorithm is very close to that of centralized optimal hybrid state estimates without sampling phase error.

==> SystemModel1.tex <==
\section{System Description} \label{sect:System-Description}
Consider first a power system module of two buses which is represented by the equivalent $\pi$ model, $i$ and $j$, connected through a branch.
The admittance at branch $\{i,j\}$ is $y_{ij}=g_{ij}+\jmath \cdot b_{ij}$, with the real and imaginary parts denoting conductance and susceptance, respectively.
Besides, denote the shunt admittance at bus $i$ as $\jmath B_i $.

The continuous voltage signal on bus $i$ at time instance $t$ is defined as  \cite{Hung2010}
\begin{equation}
\bar{E}_i(t)=E_i(t)\cos(2\pi f_c t+ \phi_i(t))
\end{equation}
Considering different PMUs are synchronized every $T_{sync}$ seconds and use imperfect local clocks with fixed clock offset $t_{i,k}$ between convective synchronization.
Let the PMU reporting time is $T$, then the voltage at bus $i$ at time instance $kT + t_{i}$
\begin{equation} \label{app-delay}
\begin{split}
\bar{E}_i(kT + t_{i,k})
&=   E_i(kT+t_{i,k})) \cos(2\pi f_c (kT + t_{i,k})+ \phi_i(kT+t_{i,k}))\\
& \approx  E_i(kT) \cos(2\pi f_c kT + \underbrace{2\pi f_c t_{i,k}}_{\triangleq\theta_{i,k}}+ \phi_i(kT)).
\end{split}
\end{equation}

We omit the index $k$ in (\ref{app-delay}) for simplicity of notion i.e. $\bar{E}_i:=\bar{E}_i(kT + t_{i,k})$ and
then the current on branch $\{i,j\}$ are given by
\begin{equation} \label{current}
\bar{I}_{ij}=(\bar{E}_i-\bar{E}_j)y_{ij} + \bar{E}_i\cdot \jmath B_i
\end{equation}


Denote the voltage in Cartesian coordinates, i.e. $E_i^r= E_p\cos (\phi_i+ \theta_i)$ $E_i^\jmath= E_i\sin (\phi_i+ \theta_i)$ and put (\ref{app-delay}) into (\ref{current}),
the delayed current are given by
\begin{equation}
\begin{split}
\bar{I}^{r}_{ij}
=&(E_i\cos (\phi_i+ \theta_i) -E_j\cos (\phi_j+ \theta_j))g_{ij}\\
&-(E_i\sin (\phi_i+ \theta_i)-E_j\sin (\phi_j+ \theta_j))b_{ij}
-B_iE_i\sin (\phi_i+ \theta_i) \\
\approx & E_i^r(g_{ij}-b_{ij}\theta_i - B_i\theta_i) + E^r_j(-g_{ij}+b_{ij}\theta_i)
+E^{\jmath}_i(-g_{ij}\theta_i-b_{ij}-B_i)+E^{\jmath}_j(g_{ij}\theta_i+b_{ij})
\end{split}
\end{equation}
\begin{equation}
\begin{split}
{I}^{\jmath}_{ij}
=&(E_i\cos (\phi_i+ \theta_i) -E_j\cos (\phi_j+ \theta_j))b_{ij}\\
&+(E_i\sin (\phi_i+ \theta_i)-E_j\sin (\phi_j+ \theta_j))g_{ij}
+B_i\cos(\phi_i+ \theta_i)  \\
\approx
& E_i^r(b_{ij}+g_{ij}\theta_i + B_i\theta_i) + E^r_j(-b_{ij}-g_{ij}\theta_i)
+E^{\jmath}_i(-b_{ij}\theta_i+g_{ij}-B_i\theta_i)+E^{\jmath}_j(b_{ij}\theta_i-b_{ij})
\end{split}
\end{equation}
As $\theta_i$ is very small (typically less than 1 degree corresponding to $46.3$ $\mu$s delay at $f_c=60$Hz), the standard approximations $\sin \theta_i \approx \theta_i $ and $\sin \theta_i \approx 1 $
With the same method, the delayed voltage can be expressed as
\begin{equation}
\bar{E}^r_{i}=E_i\cos(\phi_i+\theta_i)\approx E^r_i - E^\jmath_i\theta_i
\end{equation}
\begin{equation}
\bar{E}^\jmath_{i}=E_i\sin(\phi_i+\theta_i)\approx E^\jmath_i + E^r_i\theta_i
\end{equation}

The PMU installed on the $i^{th}$ bus measures the noisy version of
\begin{equation}
\left[\begin{array}{c}
\bar{E}^r_{i}  \\
\bar{E}^\jmath_{i}           \\
\end{array} \right]
=
\left[\begin{array}{c}
E^r_{i}          \\
E^\jmath_{i}     \\
\end{array} \right]
+ \theta_i
\left[\begin{array}{cc}
0 & -1 \\
-1& 0  \\
\end{array} \right]
\left[\begin{array}{c}
E^r_{i}          \\
E^\jmath_{i}     \\
\end{array} \right]
\end{equation}

\begin{equation}
\begin{split}
\left[\begin{array}{c}
\bar{I}^r_{ij}  \\
\bar{I}^\jmath_{ij}           \\
\end{array} \right]
=&
\left[\begin{array}{cc}
g_{ij} & -b_{ij}-B_i \\
b_{ij}+B_i& g_{ij}  \\
\end{array} \right]
\left[\begin{array}{c}
E^r_{i}          \\
E^\jmath_{i}     \\
\end{array} \right]
+
\left[\begin{array}{cc}
-g_{ij} & b_{ij} \\
-b_{ij}& -g_{ij}  \\
\end{array} \right]
\left[\begin{array}{c}
E^r_{j}          \\
E^{\jmath}_j    \\
\end{array} \right]\\
&+
\theta_i
\Bigg\{
\left[\begin{array}{cc}
-b_{ij}-B_i &  -g_{ij}\\
g_{ij}&  -b_{ij}-B_i \\
\end{array} \right]
\left[\begin{array}{c}
E^r_{i}          \\
E^\jmath_{i}     \\
\end{array} \right]
+
\left[\begin{array}{cc}
b_{ij} & g_{ij}\\
-g_{ij}& b_{ij}  \\
\end{array} \right]
\left[\begin{array}{c}
E^r_{j}          \\
E^\jmath_{j}     \\
\end{array} \right]
\Bigg\}
\end{split}
\end{equation}
The observation at bus $i$ can be written as
\begin{equation} \label{linear}
\bm z_{i}
= \sum_{j\in  \mathcal{I}(i)}  \bm H_{ij}\bm s_j
+
\theta_i\sum_{j\in  \mathcal{I}(i)}   \bm G_{ij}\bm s_j + \bm n_{i},
\end{equation}
where $\bm z_i$ is the local observations at bus $i$ which is defined as $\bm z_i = [E^r_{i}, E^\jmath_{i}, I^r_{ii_1}, I^\jmath_{ii_1},\ldots, I^r_{ii_{|\mathcal{I}(i)-1|}}, I^\jmath_{ii_{|\mathcal{I}(i)-1|}}]^T$
$\bm s_j = [E^r_{j,}, E^\jmath_{j,}]^T$
$\bm n_{i}\sim \mathcal{N}(\bm n_{i}|\bm 0, \bm R_i)$
$\mathcal{I}(i)$ is the set of all neighbors of $i$ including $i$.

The optimal estimate of state $\bm s_i$
\begin{equation}
\begin{split}
\hat{\bm s}_i =
\int...\int
&\bm s_i\prod_{i=1}^M p(\theta_i)p(\bm s_i)p(\bm R_i)
\prod_{i=1}^M
 p(\bm z_i|\theta_i, \bm s_i, \bm R_i) \\
&d\bm s_1\ldots d\bm s_{i-1}d\bm s_{i+1}\ldots d\bm s_{M}
d \theta_1\ldots d \theta_{M}
d\bm R_1\ldots d\bm R_{M}
\end{split}
\end{equation}








We omit the subscript $k$ in (\ref{app-delay}) for simplicity of notion with.  $E_i(kT):=E_i$ and
put (\ref{app-delay}) into (\ref{current}) and denote the voltage in Cartesian coordinates, i.e. $E_i^r= E_p\cos \phi_i$ $E_i^\jmath= E_p\sin \phi_i$



